DeepSpeed-VisualChat: Multi-Round Multi-Image Interleave Chat via Multi-Modal Causal Attention

Most of the existing multi-modal models, hindered by their incapacity to adeptly manage interleaved image-and-text inputs in multi-image, multi-round dialogues, face substantial constraints in resource allocation for training and data accessibility, impacting their adaptability and scalability across varied interaction realms. To address this, we present the DeepSpeed-VisualChat framework, designed to optimize Large Language Models (LLMs) by incorporating multi-modal capabilities, with a focus on enhancing the proficiency of Large Vision and Language Models in handling interleaved inputs. Our framework is notable for (1) its open-source support for multi-round and multi-image dialogues, (2) introducing an innovative multi-modal causal attention mechanism, and (3) utilizing data blending techniques on existing datasets to assure seamless interactions in multi-round, multi-image conversations. Compared to existing frameworks, DeepSpeed-VisualChat shows superior scalability up to 70B parameter language model size, representing a significant advancement in multi-modal language models and setting a solid foundation for future explorations.

==> figs/cat.tex <==
\begin{table}[!ht]
\caption{
Example visual and language inputs that demonstrate the output comparison between (1) the standard causal attention combined with cross-attention (\ca + \cra), and (2) the special multi-modal causal attention (\mmca) in \ourssingle. 
}
\label{tab:attention-comparison-cat}
% \small
\huge
\begin{adjustbox}{width=0.999\linewidth}
\centering
\begin{tabular}{p{4in}p{8in}}
\toprule
\multicolumn{2}{l}{Image and Language Inputs Example: Cat} \\ \midrule
\begin{minipage}{.95\linewidth}
\includegraphics[width=1\linewidth]{./figs/cat.png} \\
\end{minipage}                          &  {User: Please describe the image.}    \\ \midrule
\ca                                     &   The image is of \textcolor{green}{a small kitten standing on a grassy field}. The kitten is looking upwards, with its \textcolor{green}{eyes wide open, and appears to be curious about something in the sky}. The kitten is \textcolor{red}{wearing a collar} and is surrounded by green grass.      \\  \midrule
\ca + \cra                              &   The image features a cat sitting on a green lawn, with its paws stretched out in front of it. The cat is looking up and appears to be reaching for something, possibly a leaf or a flower. The grassy background provides a natural and inviting setting for the cat to explore and play.      \\  \midrule
\mmca                                   &   The image shows a cat sitting in a field of grass, surrounded by greenery. The cat is looking up and appears to be enjoying the sunshine and the outdoors. The grassy background adds to the natural setting and creates a pleasant atmosphere. The cat's expression suggests that it is content and enjoying the moment.      \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}



==> figs/ironing.tex <==
\begin{table}[!ht]
\caption{
This example illustrates the difference between \ourssingle-13B and \ourssingle-7B.
}
\label{tab:7b-13b-sculpture}
% \small
\huge
\begin{adjustbox}{width=0.999\linewidth}
\centering
\begin{tabular}{p{4in}p{8in}}
\toprule
\multicolumn{2}{l}{Image and Language Inputs Example: Ironing Man} \\ \midrule
\begin{minipage}{.95\linewidth}
\includegraphics[width=1\linewidth]{./figs/ironing.png} \\
\end{minipage}                          &   {User: What is unusual about this image?}   \\ \midrule

\ourssingle-7B                                   &    In this image, a man is standing on a busy street holding a suitcase and a parking meter.
While it is not uncommon to see people carrying suitcases, it is unusual to see someone holding a parking meter. This suggests that the man may be trying to retrieve his car from a parking spot, which is not a typical activity on a busy street. The presence of the parking meter adds an element of humor to the scene, as it is not typically seen in such a context.      \\ \midrule
\ourssingle-13B                                   &    In this image, an unusual sight is observed: a man ironing his shirt while standing on the back of a yellow taxi. This is an unconventional way of ironing one's clothes, as it is not a safe or practical method in most situations. The man is using an ironing board that is placed on the back of the taxi, and he is carefully ironing his shirt while balancing on the vehicle. This scene is likely to catch people's attention and be considered an unusual or even amusing situation.     \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> figs/lake.tex <==
\begin{table}[!ht]
\caption{
\ourssingle accurately identifies the scene as a beautiful lake and offers a set of plausible suggestions. In contrast, the baseline misinterprets the image as containing “boats”.
}
\label{tab:attention-comparison-lake}
% \small
\huge
\begin{adjustbox}{width=0.999\linewidth}
\centering
\begin{tabular}{p{4in}p{8in}}
\toprule
\multicolumn{2}{l}{Image and Language Inputs Example: Lake View} \\ \midrule
\begin{minipage}{.95\linewidth}
\includegraphics[width=1\linewidth]{./figs/lake.png} \\
\end{minipage}                          &   {User: What are the things I should be cautious about when I visit here?}   \\ \midrule
\ca                                  &   When visiting this location, which features a wooden dock \textcolor{red}{with a boat ramp} and a large body of water, you should be cautious about potential safety hazards such as slippery surfaces, uneven ground, and the possibility of falling into the water. Additionally, be aware of any boat traffic or other watercraft on the water, as well as any wildlife that may be present in the area. It is also important to follow any safety guidelines or regulations that may be in place for the dock, boat ramp, and surrounding area.      \\  \midrule
\ca + \cra                              &   When visiting the pier \textcolor{red}{with the boats} and the water, there are a few things to be cautious about. Firstly, the pier is a popular tourist spot, so it can get crowded, especially during peak seasons. It's important to be aware of your surroundings and be mindful of other people, especially if you have children with you.
Secondly, the pier is located near the water, so there is a risk of slipping or falling, especially if the surface is wet or slippery. It's recommended to wear appropriate footwear and be careful when walking on the pier.
Thirdly, the pier may have some uneven surfaces or gaps between the boards, which can be hazardous for small children or people with mobility issues. It's important to supervise children and ensure they stay on the designated pathways.
Lastly, the pier may be surrounded by water, so it's important to be aware of the tides and currents, especially if you plan to go swimming or engage in water activities. It's also important to follow any safety regulations or instructions provided by the pier or local authorities.      \\  \midrule
\mmca                                   &    When visiting this beautiful lake, I should be cautious about the following:

* The potential for slipping on the wet rocks or wooden planks that may be present around the lake.

* The possibility of encountering wildlife, such as birds or small animals, which may be present in the area.

* The potential for strong winds or sudden weather changes, which could create hazardous conditions on the water.

* The need to be aware of any safety regulations or restrictions that may be in place for the lake, such as swimming or boating restrictions.      \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> figs/sculture.tex <==

\begin{table}[!ht]
\caption{
This example illustrates the difference between \ourssingle-13B and \ourssingle-7B.
}
\label{tab:7b-13b-ironing}
% \small
\huge
\begin{adjustbox}{width=0.999\linewidth}
\centering
\begin{tabular}{p{4in}p{8in}}
\toprule
\multicolumn{2}{l}{Image and Language Inputs Example: Ironing Man} \\ \midrule
\begin{minipage}{.95\linewidth}
\includegraphics[width=1\linewidth]{./figs/sculpture.jpg} \\
\end{minipage}                          &   {User: Can you describe the image?}   \\ \midrule

\ourssingle-7B                                   &   The image shows a large sculpture of a man with a blue face and a yellow body. The man is standing on a base, and he is holding a large flower in his hand.

The sculpture is quite unique and eye-catching, with its vibrant colors and intricate details. It appears to be made of stone or some other hard material, and it is likely to be a work of art or a piece of decoration. 

The man's face is blue, and his body is yellow, which creates a striking contrast. The flower he is holding is also quite large and colorful, adding to the overall visual appeal of the sculpture. 

The sculpture is likely to be a popular attraction in a public space, such as a park or a museum, due to its unique design and vibrant colors. 

It's possible that the sculpture represents a specific character or symbol, but without further context, it's difficult to determine the exact meaning or significance of the artwork. 

Overall, the image of the blue-faced, yellow-bodied man holding a large flower is a visually striking and intriguing piece of art.      \\ \midrule
\ourssingle-13B                                   &    The image features a colorful, life-sized statue of a dog, adorned with various flowers and plants. It stands in front of a large building, possibly a stadium, with a couple of people standing nearby. One person is wearing a white shirt and is standing in front of the dog statue, while another person is standing further away to the right. The scene is vibrant and captures the attention of passersby, who are enjoying the unique artwork and the atmosphere around the building.     \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> figs/squirrel.tex <==
\begin{table}[!ht]
\caption{
\ourssingle accurately identifies the squirrel and camera in the image, while the baseline model mistakenly includes “standing next to a tree”. 
}
\label{tab:attention-comparison-quirrel}
% \small
\huge
\begin{adjustbox}{width=0.999\linewidth}
\centering
\begin{tabular}{p{4in}p{8in}}
\toprule
\multicolumn{2}{l}{Image and Language Inputs Example: Squirrel} \\ \midrule
\begin{minipage}{.95\linewidth}
\includegraphics[width=1\linewidth]{./figs/squirrel.png} \\
\end{minipage}                          &   {User: Why would a person find this image funny?}   \\ \midrule
\ca                                     &   This image is funny because it features a smiling, anthropomorphized squirrel holding a camera and taking a picture of \textcolor{red}{an apple}. The scene is playful and lighthearted, and the combination of a common everyday object like an apple with the uncommon situation of a squirrel taking a photograph adds to the humor. The squirrel's expression and the way it is depicted as taking the picture with the camera also contribute to the amusement, as it adds a sense of whimsy and creativity to the scene.      \\  \midrule
\ca + \cra                              &   The image of a smiling, well-dressed squirrel holding a camera and standing \textcolor{red}{next to a tree} is likely to be found funny because it is an unusual and unexpected combination. The juxtaposition of a cute, furry animal with a sophisticated appearance and a camera, which is typically associated with humans, creates a humorous and whimsical effect. Additionally, the squirrel's pose and expression, \textcolor{red}{along with the tree in the background}, add to the comedic effect of the image.      \\  \midrule
\mmca                                   &   A person would find this image funny because it features a cute and adorable squirrel holding a camera, which is a humorous and unexpected combination. The squirrel's expression, which is often playful and mischievous, adds to the humor, as it suggests that the squirrel is taking a picture of something or someone, possibly for its own amusement. The image also captures the quirky and whimsical nature of the squirrel, which can be entertaining and amusing to viewers. Additionally, the image's composition, with the squirrel's hand holding the camera, creates a playful and comical visual, further enhancing the humor.      \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
